Embodied Referring Expression Comprehension in Human-Robot Interaction

As robots enter human workspaces, there is a crucial need for them to comprehend embodied human instructions, enabling intuitive and fluent human-robot interaction (HRI). However, accurate comprehension is challenging due to a lack of large-scale datasets that capture natural embodied interactions in diverse HRI settings. Existing datasets suffer from perspective bias, single-view collection, inadequate coverage of nonverbal gestures, and a predominant focus on indoor environments. To address these issues, we present the Refer360 dataset, a large-scale dataset of embodied verbal and nonverbal interactions collected across diverse viewpoints in both indoor and outdoor settings. Additionally, we introduce MuRes, a multimodal guided residual module designed to improve embodied referring expression comprehension. MuRes acts as an information bottleneck, extracting salient modality-specific signals and reinforcing them into pre-trained representations to form complementary features for downstream tasks. We conduct extensive experiments on four HRI datasets, including the Refer360 dataset, and demonstrate that current multimodal models fail to capture embodied interactions comprehensively; however, augmenting them with MuRes consistently improves performance. These findings establish Refer360 as a valuable benchmark and exhibit the potential of guided residual learning to advance embodied referring expression comprehension in robots operating within human environments.

==> sections/broader_impact.tex <==
\section{Broader Impact}


==> sections/experimental_results_backup.tex <==

\section{Experimental Analysis}

% \subsection{Experimental Environment Setup}
% \label{sec:exp_setup}
% We developed all the models using the Pytorch and Pytorch-Lightning deep learning frameworks. We also used HuggingFace library for pre-trained models (BERT, ViT, Dual Encoder, and CLIP). For the Dual-Encoder and CLIP models, we used an embedding size of $512$. We train models using the Adam optimizer with a weight decay regularization set to $0$ \cite{adamw} and cosine annealing warm restarts at an initial learning rate: $3e^{-4}$, cycle length ($T_0$): $\{2,4,6\}$, and cycle multiplier ($T_{mult}$): $2$. We used batch size $32$ and trained models for $14$ epochs. We used the same fixed random seed ($33$) for all the experiments to ensure reproducibility. Lastly, all models are trained distributedly in GPU clusters, where each node contains $4$ A100 GPUs.

%We developed all the models using the Pytorch (version: 1.12.1+cu113) \cite{paszke2019pytorch} and Pytorch-Lightning (version: 1.7.1) \cite{falcon2019pytorch} deep learning frameworks. We also used HuggingFace library (version: 4.21.1) for pre-trained models (BERT \footnote{\url{https://huggingface.co/docs/transformers/model_doc/bert}} \cite{bert}, ViT \footnote{\url{https://huggingface.co/docs/transformers/model_doc/vit}} \cite{vit}, Dual Encoder \footnote{\url{https://huggingface.co/docs/transformers/model_doc/vision-text-dual-encoder}}, and CLIP \footnote{\url{https://huggingface.co/docs/transformers/model_doc/clip}} \cite{clip}). For the Dual-Encoder and CLIP models, we used an embedding size of $512$. We train models using the Adam optimizer with a weight decay regularization set to $0$ \cite{adamw} and cosine annealing warm restarts at an initial learning rate: $3e^{-4}$, cycle length ($T_0$): $\{2,4,6\}$, and cycle multiplier ($T_{mult}$): $2$. We used batch size $32$ and trained models for $14$ epochs. We used the same fixed random seed ($33$) for all the experiments to ensure reproducibility. Lastly, all models are trained in distributed GPU clusters, where each node contains $4$ A100 GPUs.

We have incorporated our proposed residual module {\pa} into the existing multimodal models, including CLIP \cite{clip}, DualEncoder \cite{wu2019dual}, ViLT \cite{kim2021vilt}, BLIP-2 \cite{li2023blip}, VisualBERT \cite{li2019visualbert}. We have evaluated these models and baselines multimodal models on {\ds} and CAESAR-PRO \cite{patron} datasets focusing on embodied referring expression comprehension ({\erfe}) tasks. We have also evaluated these models on ScienceQA \cite{lu2022learn} and A-OKVQA \cite{schwenk2022okvqa} datasets to assess their performance on Visual Question Answering (VQA) tasks. We trained multiple variations of our proposed residual module {\pa}, each differing in the type of residual representation of visual and language modalities. We examined four distinct variations:

\begin{itemize}
\item \textbf{Visual-Only Residual Representation {\pa}(V)}: This variant leverages the projected visual representation as the query in the guided residual modules to extract the salient multimodal residual representations.

\item \textbf{Language-Only Reinforced Representation {\pa}(L)}: This variant utilizes the projected language representation as the query in the guided residual modules to extract the salient multimodal residual representations.

\item \textbf{Visual and Language Reinforced Representation {\pa}(V+L)}: This variant employs projected visual and language representations as the query to extract the salient multimodal residual representations.

\item \textbf{Vanilla Residual}: Following the vanilla residual \cite{he2016deep}, This baseline directly summed visual and language to the projected representations without using any attention.
\end{itemize}

We have also evaluated several multimodal models in vanilla mode without any residual connections. All models were trained following the similar setup outlined in Section~\ref{sec:model}.

\subsection{Experimental Evaluation on Embodied Referring Expression Comprehension Task}

We evaluated the models on the {\ds} and CAESAR-PRO datasets for the embodied referring expression comprehension task. Following prior work on the embodied referring expression task \cite{chen2021yourefit}, we designed this task as an object bounding box detection task. We incorporated different variations of our multimodal guided residual module {\pa} in CLIP \cite{clip}, DualEncoder \cite{wu2019dual}, BLIP-2 \cite{li2023blip}. As ViLT \cite{kim2021vilt} is a monolithic model, we only incorporated visual-language guided residual \pa (V+L). All models were trained following the similar setup outlined in Section~\ref{sec:model} (Training Model). We reported IOU accuracy with two threshold values: $(25\%, 50\%)$. The experimental results are presented in Table~\ref{tab:vl_models_erfe}.
% \acil{Table 3 doesn't appear to have IOU-75 results; can you check?}: this is section is not completed yet


% \begin{table}[!t]
% \small
%     \centering
%     \begin{tabular}{l|cc|c|ccc}
%     \toprule
%         \multirow{2}{*}{Models} & \multicolumn{2}{c}{Reinforced Representations} & \multirow{2}{*}{Guided Reinforcement} & \multicolumn{3}{c}{Metrics} \\ \cline{2-3} \cline{5-7}
%         & Visual & Language & & IOU-25 & IOU-50 & IOU-75 \\ \hline
%         Baseline & \xmark & \xmark & \xmark & 70.05 & 41.03 & 10.40 \\
%         \rerep & \cmark & \xmark & \xmark & 70.30 & 42.50 & 11.70 \\
%         \rerep & \cmark & \cmark & \xmark & 70.30 & 43.60 & 12.30 \\
%         \rerep & \cmark & \xmark & \cmark & 72.01 & 45.79 & 12.80 \\
%         \rerep & \cmark & \cmark & \cmark & \textbf{73.49} & \textbf{51.63} & \textbf{21.21} \\
    
%     \bottomrule
%     \end{tabular}
%     \caption{Comparisons of VL models performance for object grounding task of bounding box detection on the {\ds} dataset. The results suggest that reinforcing visual and language representation in VL models can improve the performance of object ground task. We evaluated several variations of {\rerep} by varying the reinforced representations. Best performance numbers in \textbf{bold}.}
%     \label{tab:vl_models_re}
% \end{table}


% \begin{table}[!t]
% \begin{wraptable}{r}{0.55\columnwidth}
% \small
%     \centering
%     \begin{tabular}{ccccc}
%     \toprule
%         \multirow{2}{*}{\makecell{Residual\\Type}} & \multirow{2}{*}{Models} & \multicolumn{3}{c}{Metrics} \\ \cline{3-5}
%         & & IOU-25 & IOU-50 & IOU-75 \\ \hline
%         \multicolumn{5}{c}{\textbf{\ds}} \\
%         \hline
%         \multirow{4}{*}{\makecell{Without\\Residual}} & CLIP & 25.80 & 7.67 & 0.97 \\
%         & ViLT &  36.53 & 14.03 & 2.90 \\
%         & BLIP-2 &  - & - & - \\
%         & DE &  31.08 & 9.83 & 1.25 \\
%         \cline{1-5}
%         \multirow{4}{*}{\makecell{Base\\Residual\\(V+L)}} & CLIP & 27.22 & 8.35 & 1.02 \\
%         & ViLT &  35.34 & 14.37 & 3.07 \\
%         & BLIP-2 &  27.66 & 7.31 & 0.45 \\
%         & DE &  30.17 & 8.98 & 0.91 \\
%         \cline{1-5}
%          \multirow{4}{*}{\makecell{{\pa}\\(V)}} & CLIP & 29.20 & 9.15 & 0.68 \\
%         & ViLT &  - & - & - \\
%         & BLIP-2 &  25.45 & 7.71 & 1.25 \\
%         & DE &  31.36 & 8.92 & 0.91 \\
%         \cline{1-5}
%          \multirow{4}{*}{\makecell{{\pa}\\(L)}} & CLIP & 28.30 & 7.50 & 0.97 \\
%         & ViLT &  - & - & - \\
%         & BLIP-2 &  26.81 & 7.94 & 1.25 \\
%         & DE & 29.43 & 9.03 & 1.08 \\
%         \cline{1-5}
%          \multirow{4}{*}{\makecell{{\pa}\\(V+L)}} & CLIP & 26.65 & 7.27 & 0.68 \\
%         & ViLT &  37.05 & 14.66 & 2.78 \\
%         & BLIP-2 &  16.44 & 3.80 & 0.34 \\
%         & DE &  31.08 & 10.68 & 1.19 \\
%         \hline
%         \multicolumn{5}{c}{\textbf{CAESAR-PRO}} \\
%         \hline
%         \multirow{4}{*}{\makecell{Without\\Residual}} & CLIP & 37.92 & 9.82 & 0.25 \\
%         & ViLT &  27.96 & 8.73 & 0.53 \\
%         & BLIP-2 &  - & - & - \\
%         & DE &  42.52 & 12.14 & 0.28 \\
%         \cline{1-5}
%         \multirow{4}{*}{\makecell{Base\\Residual\\(V+L)}} & CLIP & 39.43 & 10.83 & 0.67 \\
%         & ViLT &  25.67 & 8.06 & 0.50 \\
%         & BLIP-2 &  30.60 & 4.92 & 0.11 \\
%         & DE &  42.61 & 11.61 & 0.81 \\
%         \cline{1-5}
%          \multirow{4}{*}{\makecell{{\pa}\\(V)}} & CLIP & 42.91 & 11.91 & 0.50 \\
%         & ViLT &  - & - & - \\
%         & BLIP-2 &  42.91 & 8.09 & 0.44 \\
%         & DE &  36.72 & 8.51 & 0.42 \\
%         \cline{1-5}
%          \multirow{4}{*}{\makecell{{\pa}\\(L)}} & CLIP & 39.56 & 10.85 & 0.70 \\
%         & ViLT &  - & - & - \\
%         & BLIP-2 &  23.85 & 3.25 & 0.11 \\
%         & DE & 37.97 & 10.32 & 0.61 \\
%         \cline{1-5}
%          \multirow{4}{*}{\makecell{{\pa}\\(V+L)}} & CLIP & 39.06 & 10.46 & 0.47 \\
%         & ViLT &  28.52 & 8.04 & 0.53 \\
%         & BLIP-2 &  38.82 & 6.75 & 0.22 \\
%         & DE &  37.72 & 11.5 & 0.81 \\
    
%     \bottomrule
%     \end{tabular}
%     \caption{Comparisons of VL models performance for object grounding task of bounding box detection on the {\ds} dataset. The results suggest that reinforcing visual and language representation in VL models can improve the performance of object ground task. We evaluated several variations of {\rerep} by varying the reinforced representations. Best performance numbers in \textbf{bold}.}
%     \label{tab:vl_models_re}
% \end{wraptable}
% \end{table}


% \begin{table}[!t]
% \centering
% \caption{Comparisons of VL models performance for object grounding task of bounding box detection. The results suggest that reinforcing visual and language representation in VL models can improve the performance of the object grounding task. We evaluated several variations by varying the reinforced representations.}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|}
% \hline
% \multicolumn{16}{c}{\textbf{\ds}} \\
% \hline
% \multirow{2}{*}{Models} & \multicolumn{3}{c|}{Without Residual} & \multicolumn{3}{c|}{Vanilla-Rep (V+L)} & \multicolumn{3}{c|}{\pa (V)} & \multicolumn{3}{c|}{\pa (L)} & \multicolumn{3}{c|}{\pa (V+L)} \\
%  & I-25 & I-50 & I-75 & I-25 & I-50 & I-75 & I-25 & I-50 & I-75 & I-25 & I-50 & I-75 & I-25 & I-50 & I-75 \\
% \hline
% CLIP & 25.80 & 7.67 & 0.97 & 27.22 & 8.35 & 1.02 & \textbf{29.20} & \textbf{9.15} & 0.68 & 28.30 & 7.50 & 0.97 & 26.65 & 7.27 & 0.68 \\
% ViLT & 36.53 & 14.03 & 2.90 & 35.34 & 14.37 & 3.07 & - & - & - & - & - & - & \textbf{37.05} & 14.66 & 2.78 \\
% BLIP-2 & - & - & - & \textbf{27.66} & 7.31 & 0.45 & 25.45 & 7.71 & 1.25 & 26.81 & 7.94 & 1.25 & 16.44 & 3.80 & 0.34 \\
% DE & 31.08 & 9.83 & 1.25 & 30.17 & 8.98 & 0.91 & \textbf{31.36} & 8.92 & 0.91 & 29.43 & 9.03 & 1.08 & 31.08 & 10.68 & 1.19 \\
% \hline
% \multicolumn{16}{c}{\textbf{CAESAR-PRO}}
% \\ \hline
% \multirow{2}{*}{Models} & \multicolumn{3}{c|}{Without Residual} & \multicolumn{3}{c|}{Vanilla-Rep (V+L)} & \multicolumn{3}{c|}{\pa (V)} & \multicolumn{3}{c|}{\pa (L)} & \multicolumn{3}{c|}{\pa (V+L)} \\
%  & I-25 & I-50 & I-75 & I-25 & I-50 & I-75 & I-25 & I-50 & I-75 & I-25 & I-50 & I-75 & I-25 & I-50 & I-75 \\
% \hline
% CLIP & 37.92 & 9.82 & 0.25 & 39.43 & 10.83 & 0.67 & \textbf{42.91} & 11.91 & 0.50 & 39.56 & 10.85 & 0.70 & 39.06 & 10.46 & 0.47 \\
% ViLT & 27.96 & 8.73 & 0.53 & 25.67 & 8.06 & 0.50 & - & - & - & - & - & - & \textbf{28.52} & 8.04 & 0.53 \\
% BLIP-2 & - & - & - & 30.60 & 4.92 & 0.11 & \textbf{42.91} & 8.09 & 0.44 & 23.85 & 3.25 & 0.11 & 38.82 & 6.75 & 0.22 \\
% DE & 42.52 & 12.14 & 0.28 & \textbf{42.61} & 11.61 & 0.81 & 36.72 & 8.51 & 0.42 & 37.97 & 10.32 & 0.61 & 37.72 & 11.5 & 0.81 \\
% \hline
% \end{tabular}%
% }
% \label{tab:horizontal_vl_models_re}
% \end{table}


\begin{table}[!t]
\centering
\caption{Comparison of VL models performance on the embodied referring expression comprehension task, designed as bounding box detection. The results suggest that our multimodal guided residual module, {\pa}, enhances the performance of most baseline multimodal models on the {\ds} and CAESAR-PRO datasets. Best performance numbers in \textbf{bold}. (V: Visual, L: Language)}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cc|cc|cc|cc|cc|}
\hline
\multicolumn{11}{c}{\textbf{{\ds} Dataset}} \\
\hline
\multirow{2}{*}{Models} & \multicolumn{2}{c|}{Without Residual} & \multicolumn{2}{c|}{Vanilla Residual} & \multicolumn{2}{c|}{\pa (V)} & \multicolumn{2}{c|}{\pa (L)} & \multicolumn{2}{c|}{\pa (V+L)} \\
 & IOU-25 & IOU-50 & IOU-25 & IOU-50 & IOU-25 & IOU-50 & IOU-25 & IOU-50 & IOU-25 & IOU-50 \\
\hline
CLIP \cite{clip} & 25.80 & 7.67 & 27.22 & 8.35 & \textbf{29.20} & \textbf{9.15} & 28.30 & 7.50 & 26.65 & 7.27 \\
ViLT \cite{kim2021vilt} & 36.53 & 14.03 & 35.34 & 14.37 & - & - & - & - & \textbf{37.05} & \textbf{14.66} \\
BLIP-2 \cite{li2023blip} & - & - & \textbf{27.66} & 7.31 & 25.45 & 7.71 & 26.81 & \textbf{7.94} & 16.44 & 3.80 \\
Dual-Encoder \cite{wu2019dual} & 31.08 & 9.83 & 30.17 & 8.98 & \textbf{31.36} & 8.92 & 29.43 & 9.03 & 31.08 & \textbf{10.68} \\
% Dual-Encoder \cite{wu2019dual} & 70.05 & 41.03 & 70.30 & 43.60 & \textbf{72.01} & 45.79 & 70.30 & 42.50 & 73.49 & \textbf{51.63} \\
\hline
\multicolumn{11}{c}{\textbf{CAESAR-PRO Dataset \cite{patron}}} \\
\hline
\multirow{2}{*}{Models} & \multicolumn{2}{c|}{Without Residual} & \multicolumn{2}{c|}{Vanilla Residual} & \multicolumn{2}{c|}{\pa (V)} & \multicolumn{2}{c|}{\pa (L)} & \multicolumn{2}{c|}{\pa (V+L)} \\
 & IOU-25 & IOU-50 & IOU-25 & IOU-50 & IOU-25 & IOU-50 & IOU-25 & IOU-50 & IOU-25 & IOU-50 \\
\hline
CLIP \cite{clip} & 37.92 & 9.82 & 39.43 & 10.83 & \textbf{42.91} & \textbf{11.91} & 39.56 & 10.85 & 39.06 & 10.46 \\
ViLT \cite{kim2021vilt} & 27.96 & \textbf{8.73} & 25.67 & 8.06 & - & - & - & - & \textbf{28.52} & 8.04 \\
BLIP-2 \cite{li2023blip} & - & - & 30.60 & 4.92 & \textbf{42.91} & \textbf{8.09} & 23.85 & 3.25 & 38.82 & 6.75 \\
Dual-Encoder \cite{wu2019dual} & 42.52 & \textbf{12.14} & \textbf{42.61} & 11.61 & 36.72 & 8.51 & 37.97 & 10.32 & 37.72 & 11.5 \\
\hline
\end{tabular}%
}
\label{tab:vl_models_erfe}
\end{table}







\textbf{Results and Discussion: } The experimental results in Table~\ref{tab:vl_models_erfe} indicate that augmenting multimodal guided residual module {\pa} into multimodal models enhances embodied referring expression comprehension task performance on both the {\ds} and CAESAR-PRO datasets. Specifically, the experimental results in Table~\ref{tab:vl_models_erfe} indicate that including visual reinforced representation enhances task performance. For example, augmenting {\pa} into CLIP\cite{clip} model and reinforcing visual representation improved object bounding detection task performance on our {\pa} dataset from $25.80\%$ to $29.20\%$ for IOU-25. Similarly, {\pa} helps CLIP\cite{clip} model enhance object bounding detection task performance on CAESAR-PRO \cite{patron} dataset from $37.92\%$ to $42.91\%$ for IOU-25. This performance improvement underscores the importance of visual cues in object grounding and suggests that reinforcing visual representation can lead to better performance. 

Although the vanilla residual connection offers some performance improvement over models without any residual connection-based fusion, the gains are modest compared to those achieved with {\pa}. The key distinction lies in {\pa}'s selective reinforcement of the most salient aspects of the visual-language representation, acting as an information bottleneck to extract only the relevant information. This targeted approach contrasts with vanilla residual connections, which indiscriminately reinforce the entire representation. These insights align with the findings from prior works on the information bottleneck. In the literature, it has been shown that information bottleneck helps the model to extract the relevant information and thus improve downstream task performance. Thus, the design choice of residual representation incorporation is pivotal in refining multimodal representation and, consequently, downstream task performance.

% However, although vanilla residual connection \cite{he2016deep} improves the performance compared to the multimodal without any residual connection-based fusion, this performance improvement is slight compared to {\pa}. The primary reason behind this performance discrepancy is that vanilla residual connections reinforce complete representation without identifying the salient part of the representations. Conversely, {\pa} works as an information bottleneck and extracts only the relevant part of the visual-language representation, which needs to be reinforced. This guided residual can help to improve the multimodal representation and thus improve the downstream task performance. These findings also align with the existing literature on the information bottleneck. In the literature, it has been shown that information bottleneck helps extract the relevant information and thus improve downstream task performance. Thus, how we incorporate the residual representation impacts multimodal representation and downstream task performance.

The experimental results further suggest that the specific modality being reinforced significantly influences performance improvements. For example,  reinforcing the visual modality with {\pa} boosts the CLIP model's performance for the object bounding box detection task from $25.80\%$ to $29.20\%$ for IOU-25. Conversely, emphasizing the language modality results in a slightly lower enhancement, with performance increasing to $28.30\%$. This variance suggests that the object grounding task is predominantly reliant on visual information. Thus, the choice of modality for reinforcement should be carefully considered based on the downstream task.

% reinforcing visual modality using {\pa} helps to improve the performance of CLIP model for object bounding box detection from $25.80\%$ to $29.20\%$ for IOU-25 whereas reinforcing language modality in {\pa} helps to improve the performance of CLIP model to $28.30$. The reasoning behind the performance degradation with reinforced language modality is that object grounding task highly depends on the visual modality. Thus, which modality should we reinforce depends on the task. 

% The results further indicate that incorporating both visual and language representations as reinforced representations can significantly enhance the performance of the object grounding task. For example, our proposed model, {\rerep}, which utilizes both visual and language representation, boosts the baseline model performance by a notable $3.45\%$ for IOU-25. This outcome underscores the multimodal aspect of the task and implies that a balanced approach to both visual and language cues can result in more precise object grounding. Furthermore, equipped with reinforced representations, our proposed model {\rerep} consistently surpasses the baseline across all IOU thresholds. This experimental result validates our proposed model's effectiveness and highlights the significance of reinforced representations in extracting pertinent features for object grounding tasks.


% While our proposed model, {\rerep}, shows modest improvements in task performance at lower IOU thresholds ($25\%$ and $50\%$), it demonstrates a significant performance boost at higher IOU thresholds. Specifically, {\rerep} achieves a $10.81\%$ improvement in the bounding box prediction task at higher IOU thresholds. This is particularly noteworthy as achieving high performance at higher IOU thresholds is challenging. IOU, or Intersection over Union, is a metric used to evaluate the accuracy of an object detector on a specific dataset. Higher IOU thresholds are more challenging because they require the predicted bounding box to match the ground truth bounding box more closely. In other words, a model must correctly identify the objects with high precision to achieve a high score at these thresholds. The significant improvement achieved by {\rerep} at these thresholds suggests that our model is particularly effective at accurately identifying objects, even under stringent evaluation criteria.

% However, our analysis also reveals the crucial role of guided reinforcement in our model's performance. Without the use of guided reinforcement, our model's performance drops by $8.91\%$ for IOU-75. This drop in performance underscores the importance of guided reinforcement in our proposed approach. Guided reinforcement helps the model focus on the most relevant parts of the input, thereby improving the quality of the reinforced representations. It essentially guides the learning process, helping the model to better leverage the reinforced representations for the task at hand. Our detailed analysis highlights the effectiveness of our proposed model, {\rerep}, particularly at higher IOU thresholds. It also emphasizes the importance of guided reinforcement in enhancing the model's performance. These findings provide valuable insights for developing effective visual-language representation learning models.

% The experimental results also indicate that multimodal reinforced representations can effectively supplement the aligned representations derived using the self-attention approach. This observation suggests that while the self-attention mechanism is adept at aligning visual and language modalities, incorporating reinforced representations can offer a more refined balance between these modalities, leading to enhanced task performance.

% Therefore, our experimental analysis showcases the potential of reinforced representations in augmenting the performance of object grounding tasks. It also underscores the necessity for models capable of dynamically adjusting the balance between visual and language modalities, contingent on the specific requirements of the task at hand.


% The experimental results in Table~\ref{tab:vl_models_patron} suggest that incorporating the visual reinforced representation helps to improve the performance of the bounding box detection task from $70.05\%$ to $72.05\%$ for IOU-25. This performance improvement indicates the importance of reemphasizing visual representation for object grounding. However, if we use reinforced representation without guided reinforcement then the model's performance improved slightly by $0.25\%$ for IOU-25. This signifies the importance of using visual reinforced representation through guided reinforcement.

% Similarly, utilizing visual and language representations can help improve the object grounding task performance further. For example, {\rerep} with visual and language representation can improve the baseline model performance by $3.45\%$ for IOU-25. Although our model {\rerep} slightly improves the task performance for lower thresholds of IOUs ($25\% and 50\%$), for higher IOU thresholds, which is very challenging, {\rerep} can achieve $10.81\%$ improvement for bounding box prediction task. IOU with a higher threshold is challenging as it evaluates whether the model can appropriately identify the objects appropriately. However, if we do not use guided reinforcement, then our model performance drops by $8.91$. This emphasizes the importance of our proposed guided reinforced representation-based visual-language representation learning.

% Our proposed model {\rerep} with reinforced representations can help to improve the object grounding task performance across all the IOU thresholds. The experimental results suggest the effectiveness of reinforced representation in extracting salient representation for object grounding tasks. Multimodal reinforced representations complement the aligned representations extracted using the self-attention approach. 


% \begin{table}[!t]
% \small
%     \centering
%     \begin{tabular}{lccc}
%     \toprule
%         \multirow{2}{*}{Models} & \multicolumn{3}{c}{Metrics} \\ \cline{2-4} 
%         & IOU-25 & IOU-50 & IOU-75 \\ \hline
%         DualEncoder  & 31.08 & 10.68 & 1.19 \\
%         CLIP  & 27.22 & 8.35 & 1.02 \\
%         ViLT & 35.34 & 14.37 & 3.07 \\
%         BLIP-2 & 13.95 & 2.04 & 0.06 \\
%         \rerep & \textbf{73.49} & \textbf{51.63} & \textbf{21.21} \\
    
%     \bottomrule
%     \end{tabular}
%     \caption{Comparisons of VL models performance for object grounding task of bounding box detection on the {\ds} dataset. The results suggest that reinforcing visual and language representation in VL models can improve the performance of object ground task. We evaluated several variations of {\rerep} by varying the reinforced representations. Best performance numbers in \textbf{bold}.}
%     \label{tab:vl_models_re}
% \end{table}




\subsection{Experimental Evaluation on Visual Question-Answering Task}

% We have conducted the experimental analysis on our CAESAR-PRO dataset \cite{patron}. We trained several variations of our proposed model by varying the reinforced representation of visual and language representations. We varied the reinforced representation in three ways: using only visual representation as reinforced representation, using only language representation as reinforced representation, and using visual and language representations as reinforced representation. We also used guided attention to extract the reinforced representations. We trained the baseline Dual-Encoder model on the CAESAR-PRO dataset. We extract the visual and language representations using the pretrained model for Dual-Encoder models. The visual and language representations are summed to produce the task representation for the bounding box detection task.

We conducted experimental analysis on the CAESAR-PRO dataset \cite{patron}. Through this detailed experimental analysis, we aimed to evaluate the effectiveness of our proposed model and its variations compared to the baseline model. Similar to the experimental evaluation on {\ds}, we trained several variations of our proposed model by varying the reinforced representation of visual and language representations. We explored three distinct variations in the reinforced representation: Visual-Only Reinforced Representation, Language-Only Reinforced Representation, Visual and Language Reinforced Representation.

% \begin{enumerate}
%     \item \textbf{Visual-Only Reinforced Representation}: In this variant, we solely used the visual representation as the reinforced representation. This approach emphasizes the importance of visual cues in the task of object bounding box prediction.
%     \item \textbf{Language-Only Reinforced Representation}: In this variant, we exclusively used the language representation as the reinforced representation. This approach underscores the significance of language cues in the task.
%     \item \textbf{Visual and Language Reinforced Representation}: In this variant, we used both visual and language representations as the reinforced representation. This approach recognizes the multimodal nature of the task and attempts to balance the contributions of both visual and language cues.
% \end{enumerate}

In some variations, we employed guided attention to extracting the reinforced representations. Guided attention helps the model focus on the most relevant parts of the input, thereby improving the quality of the reinforced representations.

As a baseline, we trained the Dual-Encoder model on the CAESAR-PRO dataset. We used a pretrained Dual-Encoder model from the HuggingFace library to extract the visual and language representations. These representations were then summed to produce the task representation for the bounding box detection task.

We trained all the models following the similar setup presented in Section~\ref{sec:exp_setup}. Following the prior work \cite{chen2021yourefit}, we have reported IOU accuracy with various thresholds values $(25\%, 50\%, 75\%)$. The experimental results are presented in Table~\ref{tab:vl_models_patron}.

% Through this detailed experimental analysis, we aimed to evaluate the effectiveness of our proposed model and its variations. The results of this analysis provide valuable insights into the role of reinforced representations in the task of object bounding box prediction.

% \begin{table}[!t]
% \small
%     \centering
%     \begin{tabular}{l|cc|c|ccc}
%     \toprule
%         \multirow{2}{*}{Models} & \multicolumn{2}{c}{Reinforced Representations} & \multirow{2}{*}{Guided Reinforcement} & \multicolumn{3}{c}{Metrics} \\ \cline{2-3} \cline{5-7}
%         & Visual & Language & & IOU-25 & IOU-50 & IOU-75 \\ \hline
%         Baseline & \xmark & \xmark & \xmark & 46.60 & 13.84 & 1.26 \\
%         \rerep & \cmark & \xmark & \xmark & 51.60 & 20.40 & 2.30 \\
%         \rerep & \cmark & \cmark & \xmark & \textbf{55.51} & \textbf{21.70} & \textbf{2.70} \\
    
%     \bottomrule
%     \end{tabular}
%     \caption{Comparisons of VL models performance for object grounding task of bounding box detection on the CAESAR-PRO dataset. The results suggest that reinforcing visual and language representation in VL models can improve the performance of object ground task. We evaluated several variations of {\rerep} by varying the reinforced representations. Best performance numbers in \textbf{bold}.}
%     \label{tab:vl_models_patron}
% \end{table}


% \begin{table}[!t]
% \begin{wraptable}{r}{0.45\columnwidth}
% \small
%     \centering
%     \begin{tabular}{ccc}
%     \toprule
%         \makecell{Residual\\Type} & Models & Accuracy \\ 
%         \hline
%         \multicolumn{3}{c}{ScienceQA \cite{lu2022learn}} \\
%         \hline
%         \multirow{3}{*}{\makecell{Base\\Residual\\(V+L)}} & CLIP & 71.38 \\
%         & ViLT & 62.25 \\
%         & VisualBERT & 62.76 \\
%         \cline{1-3}
%         \multirow{3}{*}{\makecell{{\pa}\\(V)}} & CLIP & 73.21 \\
%         & ViLT & 65.07 \\
%         & VisualBERT & 66.29 \\
%         \cline{1-3}
%         \multirow{3}{*}{\makecell{{\pa}\\(L)}} & CLIP & 72.63 \\
%         & ViLT & 64.34 \\
%         & VisualBERT & 64.55 \\
%         \cline{1-3}
%         \multirow{3}{*}{\makecell{{\pa}\\(V+L)}} & CLIP & 73.94 \\
%         & ViLT & 66.78 \\
%         & VisualBERT & 67.34 \\
        
%         \hline
%         \multicolumn{3}{c}{AOKVQA \cite{schwenk2022okvqa}} \\
%         \hline
%         \multirow{3}{*}{\makecell{Base\\Residual\\(V+L)}} & CLIP & 51.29 \\
%         & ViLT & 41.06 \\
%         & VisualBERT & 41.58 \\
%         \cline{1-3}
%         \multirow{3}{*}{\makecell{{\pa}\\(V)}} & CLIP & 52.07 \\
%         & ViLT & 42.88 \\
%         & VisualBERT & 43.36 \\
%         \cline{1-3}
%         \multirow{3}{*}{\makecell{{\pa}\\(L)}} & CLIP & 51.66 \\
%         & ViLT & 42.20 \\
%         & VisualBERT & 42.53 \\
%         \cline{1-3}
%         \multirow{3}{*}{\makecell{{\pa}\\(V+L)}} & CLIP & 52.83 \\
%         & ViLT & 43.92 \\
%         & VisualBERT & 44.14 \\
    
%     \bottomrule
%     \end{tabular}
%     \caption{Comparisons of VL models performance for object grounding task of bounding box detection on the respective datasets. The results suggest that reinforcing visual and language representation in VL models can improve the performance of object grounding tasks. We evaluated several variations of reinforced representations. Best performance numbers in \textbf{bold}.}
%     \label{tab:vl_models_re}
% \end{wraptable}


% \end{table}

\begin{table}[!t]
% \begin{wraptable}{r}{0.65\columnwidth}
\small
\centering
% \caption{Comparisons of VL models performance for object grounding task of bounding box detection on the respective datasets. The results suggest that reinforcing visual and language representation in VL models can improve the performance of object grounding tasks. We evaluated several variations of reinforced representations. Best performance numbers in \textbf{bold}.}
\caption{Comparison of VL models performance on the visual question-answering task. The results suggest that our multimodal guided residual module, {\pa}, enhances the performance of the multimodal models on the ScienceQA and A-OKVQA datasets. Best performance numbers in \textbf{bold}. (V: Visual, L: Language)}

\begin{tabular}{|l|c|c|c|c|}
\hline
\multicolumn{5}{|c|}{\textbf{ScienceQA Dataset \cite{lu2022learn}}} \\ \hline
Models & Without Residual & \pa (V) & \pa (L) & \pa (V+L) \\ \hline
CLIP \cite{clip} & 71.38 & 73.21 & 72.63 & \textbf{73.94} \\
ViLT \cite{kim2021vilt} & 62.25 & 65.07 & 64.34 & \textbf{66.78} \\
VisualBERT \cite{li2019visualbert} & 62.76 & 66.29 & 64.55 & \textbf{67.34} \\ \hline
\bottomrule
\multicolumn{5}{|c|}{\textbf{A-OKVQA Dataset \cite{schwenk2022okvqa}}} \\ \hline
Models & Without Residual & \pa (V) & \pa (L) & \pa (V+L) \\ \hline
CLIP \cite{clip} & 51.29 & 52.07 & 51.66 & \textbf{52.83} \\
ViLT \cite{kim2021vilt} & 41.06 & 42.88 & 42.20 & \textbf{43.92} \\
VisualBERT \cite{li2019visualbert} & 41.58 & 43.36 & 42.53 & \textbf{44.14} \\
\hline
\end{tabular}
\label{tab:vl_models_scienceqa_aokvqa}
% \end{wraptable}

\end{table}


% \textbf{Results and Discussion: } The experimental results, as presented in Table~\ref{tab:vl_models_patron}, show the effectiveness of reinforced representations for object bounding box prediction task. The results indicate that including visual reinforced representation enhances the task performance, improving from $46.60\%$ to $51.60\%$ for IOU-25. This enhancement underscores the importance of visual cues in object grounding and suggests that reemphasizing visual representation can lead to better performance.

% Interestingly, the results also show that using both visual and language representations as reinforced representations can further boost the performance of the object grounding task. For instance, with both visual and language representation, our proposed model, {\rerep}, improves the baseline model performance by a substantial $8.91\%$ for IOU-25. This finding highlights the multimodal nature of the task and suggests that a balanced consideration of both visual and language cues can lead to more accurate object grounding. Moreover, our proposed model {\rerep} with reinforced representations consistently outperforms the baseline across all IOU thresholds. This result validates our proposed model's effectiveness and emphasizes the importance of reinforced representations in extracting salient features for object grounding tasks.

% The experimental results also suggest that multimodal reinforced representations complement the aligned representations extracted using the self-attention approach. This finding indicates that while the self-attention mechanism effectively aligns visual and language modalities, the addition of reinforced representations complements the aligned representations, leading to improved task performance.

% In conclusion, our experimental analysis demonstrates the potential of reinforced representations in improving the performance of object grounding tasks. It also highlights the need for models that can dynamically adjust the balance between visual and language modalities based on the specific requirements of the task at hand. These insights pave the way for future research in this exciting field of comprehending embodied interactions.


% The experimental results in Table~\ref{tab:vl_models_patron} suggest that incorporating the visual reinforced representation helps to improve the performance of the bounding box detection task from $46.60\%$ to $51.60\%$ for IOU-25. This performance improvement indicates the importance of reemphasizing visual representation for object grounding. Most importantly, utilizing visual and language representations can help improve the object grounding task performance further. For example, {\rerep} with visual and language representation can improve the baseline model performance by $8.91\%$ for IOU-25. Our proposed model {\rerep} with reinforced representations can help to improve the object grounding task performance across all the IOU thresholds. The experimental results suggest the effectiveness of reinforced representation in extracting salient representation for object grounding tasks. Multimodal reinforced representations complement the aligned representations extracted using the self-attention approach. 

==> sections/limitations.tex <==
\section{Limitations and Future Works}

